Computing the log-determinant of symmetric, diagonally dominant matrices in near-linear time

We present new algorithms for computing the log-determinant of symmetric, diagonally dominant matrices. Existing algorithms run with cubic complexity with respect to the size of the matrix in the worst case. Our algorithm computes an approximation of the log-determinant in time near-linear with respect to the number of non-zero entries and with high probability. This algorithm builds upon the utra-sparsifiers introduced by Spielman and Teng for Laplacian matrices and ultimately uses their refined versions introduced by Koutis, Miller and Peng in the context of solving linear systems. We also present simpler algorithms that compute upper and lower bounds and that may be of more immediate practical interest.

==> detsdd_6bounds.tex <==

\section{Structural bounds on the log-determinant}

How good is the estimate provided by the tree $T$? Intuitively, this
depends on how well the tree $T$ approximates the graph $G$. This
notion of quality of approximation can be formalized by the notion
of \emph{stretch}. \begin{definition} Stretch of a graph. Consider
$G$ a weighted graph, and $T$ a spanning tree of $G$. The stretch
of each edge $e$ from $G$ is defined as $\text{st}_{T}\left(e\right)=\omega_{e}\left(\sum_{f\in P}\frac{1}{\omega_{f}}\right)$
where $\omega_{e}$ is the weight of edge $e$ in $G$, and $P$ is
the unique path between the endpoints of $e$ in the tree $T$. The
stretch of the graph is the sum of the stretches of each edge: 
\[
\text{st}_{T}\left(G\right)=\sum_{e\in G}\text{st}_{T}\left(e\right)
\]


\end{definition} The stretch can be obtained as a by-product of the
computation of low-stretch spanning trees, of which the construction
can be done in $O\left(m\log n+n\log^{2}n\right)$ \cite{Abraham2008}.
Knowing the stretch gives upper and lower bounds on the value of the
log-determinant. \begin{proposition} Stretch bounds on the tree PLD:
\end{proposition} 
\begin{equation}
\log\left|T\right|+\left(n-1\right)\log\left(\frac{\text{st}_{G}\left(T\right)}{n-1}\right)\geq\log\left|G\right|\geq\log\left|T\right|+\log\left(\text{st}_{T}\left(G\right)-n+2\right)\label{eq:encadrement}
\end{equation}


\begin{proof} This is an application of Jensen's inequality on $\text{ld}\left(T^{+}G\right)$.
We have $\text{ld}G=\text{ld}T+\text{ld}\left(T^{+}G\right)$ and
$\text{ld}\left(T^{+}G\right)=\text{ld}\left(\sqrt{T}^{+}G\sqrt{T}^{+}\right)=\text{Tr}\left(\log^{+}\left(\sqrt{T}^{+}G\sqrt{T}^{+}\right)\right)$
with $\sqrt{T}$ the matrix square root of $T$. From Lemma \ref{lem:Jensen-inequality-matrix-logarithm},
we have 
\begin{eqnarray*}
\text{Tr}\left(\log^{+}\left(\sqrt{T}^{+}G\sqrt{T}^{+}\right)\right) & \leq & \left(n-1\right)\log\left(\frac{\text{Tr}\left(\sqrt{T}^{+}G\sqrt{T}^{+}\right)}{n-1}\right)\\
 & = & \left(n-1\right)\log\left(\frac{\text{Tr}\left(T^{+}G\right)}{n-1}\right)\\
 & = & \left(n-1\right)\log\left(\frac{\text{st}_{G}\left(T\right)}{n-1}\right)
\end{eqnarray*}


The lower bound is slightly more involved. Call $\lambda_{i}$ the
positive eigenvalues of $\sqrt{T^{+}}G\sqrt{T^{+}}$ and $\sigma=\text{st}_{T}\left(G\right)$.
We have $1\leq\lambda_{i}\leq\sigma$ because of the inequality$T\preceq G\preceq\text{st}_{T}\left(G\right)T$.
There are precisely $n-1$ positive eigenvalues $\lambda_{i}$, and
we have: $\text{ld}\left(T^{+}G\right)=\sum_{i}\log\lambda_{i}$.
One can show that $\sum_{i}\log\lambda_{i}\geq\log\left(\sigma-n+2\right)$
by considering the problem of minimizing $\sum_{i}\log x_{i}$ under
the constraints $\sum_{i}x_{i}=\sigma$ and $x_{i}\geq1$. This bound
is tight. \end{proof} Intuitively since the stretch of a tree is
bounded my $O\left(m\log n\right)$, it means that a low-stretch spanning
tree provides an approximation of a log-determinant up to a factor
of $O\left(n\log n\right)$. This could be of interest for nearly-cut
graphs, with large condition numbers.



\begin{lemma} \label{lem:Jensen-inequality-matrix-logarithm}Jensen
inequality for the matrix logarithm. Given $A\in\mathcal{S}_{n}^{+},$
$0\prec A\prec2$, the following inequalities hold: 
\[
\log\left(\frac{\text{Tr}\left(A\right)}{n}\right)\geq\frac{1}{n}\text{Tr}\left(\log A\right)
\]
\[
\text{ld}\left(\frac{\text{Tr}\left(A\right)}{n-1}\right)\geq\frac{1}{n-1}\text{Tr}\left(\log A\right)
\]
with $\log A=\sum_{k\geq1}\frac{1}{k}\left(I-A\right)^{k}$\end{lemma}
\begin{proof} Consider the diagonalization of $A$: $A=P\Delta P^{T}$
with $\Delta$ a diagonal (positive) matrix, and $P$ an orthogonal
matrix. Then 
\[
\log A=\sum_{k\geq1}\frac{1}{k}\left(PP^{T}-P\Delta P^{T}\right)^{k}=\sum_{k\geq1}\frac{1}{k}\left[P\left(I-\Delta\right)P^{T}\right]^{k}=P\left[\sum_{k\geq1}\frac{1}{k}\left(I-\Delta\right)^{k}\right]P^{T}=P\Gamma P^{T}
\]
with $\Gamma$ a diagonal matrix that verifies $\Gamma_{ii}=\log\Delta_{ii}$.
We can then conclude using the concavity of the logarithm over the
reals: 
\[
\log\left(\frac{\text{Tr}\left(A\right)}{n}\right)=\log\left(\frac{\sum_{i}\Delta_{ii}}{n}\right)\geq\frac{1}{n}\sum_{i}\log\Delta_{ii}=\frac{1}{n}\text{Tr}\left(\Gamma\right)=\frac{1}{n}\text{Tr}\left(\log A\right)
\]


The same reasoning holds for the pseudo-log-determinant while considering
all but one eigenvalue\end{proof} \begin{lemma} Power relation for
the matrix log: Given $A\in\mathcal{S}_{n}^{+},$ $0\prec A\prec2$,
and $k\in\mathbb{N}$, then $\log\left(A^{k}\right)=k\log A$ \end{lemma}


\subsection{Stretch of a graph\label{sub:Stretch-graph}}

We introduce here a refinement on an upper bound that is a byproduct
of using the algorithm XXX. \begin{definition} We define the \textbf{stretch
of a graph} $G=\left(V,E,\omega\right)$ with respect to a subgraph
$H=\left(V,\tilde{E},\tilde{\omega}\right)\subset G$ by the weighted
sum of effective resistances of edges $e\in E$ with respect to the
graph $H$: 
\[
\text{st}_{H}\left(G\right)=\sum_{e\in E}\omega_{e}\text{eff}_{H}\left(e\right)
\]


\end{definition} This is a generalization of the notion of stretch
defined by Alon, Karp, Peleg and West in .... We can use this definition
to generalize theorem 2.1 in \cite{Spielman2009b} \begin{theorem}
Let $G=\left(V,E,\omega\right)$ be a connected graph and let $H=\left(V,\tilde{E},\tilde{\omega}\right)$
be a connected subgraph of $G$. Let $L_{G}$ and $L_{H}$ be the
Laplacian matrices of $G$ and $H$ respectively. Then: 
\[
\text{Tr}\left(L_{H}^{+}L_{G}\right)=\text{st}_{H}\left(G\right)
\]
where $L_{H}^{+}$ is the pseudo inverse of $L_{H}$.\end{theorem}
\begin{proof} The proof is nearly identical to that of \cite{Spielman2009b},
except for the last line:

\begin{eqnarray*}
\text{Tr}\left(L_{H}^{+}L_{G}\right) & = & \sum_{\left(u,v\right)\in E}\omega\left(u,v\right)\text{Tr}\left(L_{\left(u,v\right)}L_{H}^{+}\right)\\
 & = & \sum_{\left(u,v\right)\in E}\omega\left(u,v\right)\text{Tr}\left(\left(\psi_{u}-\psi_{v}\right)\left(\psi_{u}-\psi_{v}\right)^{T}L_{H}^{+}\right)\\
 & = & \sum_{\left(u,v\right)\in E}\omega\left(u,v\right)\left(\psi_{u}-\psi_{v}\right)^{T}L_{H}^{+}\left(\psi_{u}-\psi_{v}\right)
\end{eqnarray*}
and the latter term is the effective resistance between $u$ and $v$
in the graph $H$: 
\begin{eqnarray*}
 & = & \sum_{\left(u,v\right)\in E}\omega\left(u,v\right)\text{eff}_{H}\left(u,v\right)\\
 & = & \text{st}_{H}\left(G\right)
\end{eqnarray*}


\end{proof} From a practical perspective, the graph stretch can be
computed in $\tilde{O}\left(m\log n/\epsilon^{2}\right)$ \begin{proposition}
There exists an algorithm that computes an $\epsilon$-approximation
of $\text{st}_{H}\left(G\right)$ in $\tilde{O}\left(m\log n/\epsilon^{2}\right)$\end{proposition}
\begin{proof} This is the second main result from Spielman and Srivastana
(XXX cite). \end{proof}

